Thrust Regulation Through Wing Linkage Modulation on the Aerobat Platform: Piezoelectric Slip-Stick Actuated Regulator Development

Aerobat is a bat-inspired flapping-wing robot with a wing gait generate by the computational structure, a planar linkage of carbon fiber links driven by a single motor. This design minimizes weight but couples both wings to a shared input motor, eliminating independent thrust control and preventing asymmetric maneuvers. This thesis investigates thrust regulation by modifying the effective length of the first radius link $R_1$ in the computational structure. Static experiments using FDM-printed $R_1$ links at three lengths (28.58, 29.33, and 30.08 mm) across 3,4, and 5 Hz flapping frequencies demonstrated that a 1.5 mm length increase produced a 37% increase in peak lift force and shifted peak force timing within the downstroke. An additional experiment using a string-actuated regulator mechanism was performed. Further actuation methods were evaluated: sub-gram micro-servo and piezoelectric slip-stick. After both the string-tension and micro-servo actuation methods failed due to structural member compliance and motor fragility respectively, a TULA-50 piezoelectric slip-stick actuator was selected. Multiple force-amplifying mechanisms were prototyped, resulting in a direct-drive variable-length mechanism. This final mechanism was demonstrated in a preliminary bench-top test, though insufficient force output prevented dynamic testing during flapping. This work establishes linkage-length modulation via embedded slip-stick actuation as a viable approach to independent wing thrust control.

==> tex/dedication.tex <==
% dedication.tex:

\begin{dedication}
To my family.
\end{dedication}

